Sample Efficient Ensemble Learning with Catalyst.RL

We present Catalyst.RL, an open-source PyTorch framework for reproducible and sample efficient reinforcement learning (RL) research. Main features of Catalyst.RL include large-scale asynchronous distributed training, efficient implementations of various RL algorithms and auxiliary tricks, such as n-step returns, value distributions, hyperbolic reinforcement learning, etc. To demonstrate the effectiveness of Catalyst.RL, we applied it to a physics-based reinforcement learning challenge "NeurIPS 2019: Learn to Move -- Walk Around" with the objective to build a locomotion controller for a human musculoskeletal model. The environment is computationally expensive, has a high-dimensional continuous action space and is stochastic. Our team took the 2nd place, capitalizing on the ability of Catalyst.RL to train high-quality and sample-efficient RL agents in only a few hours of training time. The implementation along with experiments is open-sourced so results can be reproduced and novel ideas tried out.

==> text/2_related.tex <==
\section{Related work}\label{sec:related}

\paragraph{Reproducibility} In recent years, a lot of concerns about reproducibility of deep reinforcement learning (RL) algorithms have been raised. \cite{islam2017reproducibility} investigated recent advances in policy gradient algorithms for continuous control and came to the conclusion that claimed state-of-the-art results are difficult to reproduce due to general variance in algorithms and extreme sensitivity to hyper-parameter tuning. Later, this analysis was extended by \cite{henderson2018deep}, which showed that entirely different levels of performance might be achieved by the same algorithms if taken from different codebases. They also investigated common flaws in reporting evaluation metrics and provided recommendations on their improvement. \cite{machado2018revisiting} analyzed the diversity of evaluation methodologies in Arcade Learning Environment and highlighted some key concerns and best practices for reporting the experimental results. Recently, \cite{colas2018many} has proposed to look at reproducibility in deep RL through the lens of statistical hypothesis testing and \cite{nagarajan2018deterministic} has investigated the effects of different sources of non-determinism on the performance of deep Q-learning algorithm.

\paragraph{Codebases} In order to fight reproducibility crisis and make recent advances in deep RL more accessible to the wider audience, a large number of codebases have been released. \cite{duan2016benchmarking} conducted an extensive comparison of popular deep RL algorithms for continuous control implemented in \textit{rllab}\footnote{\url{https://github.com/rll/rllab}} framework. OpenAI presented \texttt{Baselines}\footnote{\url{https://github.com/openai/baselines}}, reference implementations of various RL algorithms, and \texttt{Spinning Up}\footnote{\url{https://github.com/openai/spinningup}}, an educational resource aimed to lower the entry threshold into RL research. 
\cite{liang2018rllib} introduced \texttt{RLLib}\footnote{\url{https://github.com/ray-project/ray/tree/master/python/ray/rllib}}, an open-source library for RL that offered both a collection of reference algorithms and scalable primitives for composing new ones. \cite{castro2018dopamine} presented \texttt{Dopamine}\footnote{\url{https://github.com/google/dopamine}}, a research framework for fast prototyping of reinforcement learning algorithms in \texttt{TensorFlow}. \cite{schaarschmidt2018rlgraph} released \texttt{RLGraph}, a library for designing and executing high performance RL computation graphs in both static graph and define-by-run paradigms. 
Recently, \cite{gauci2018horizon} has introduced \texttt{Horizon}\footnote{\url{https://github.com/facebookresearch/Horizon}}, Facebook's open source applied RL platform, and \cite{fan2018surreal} presented \texttt{Surreal}\footnote{\url{https://github.com/SurrealAI/surreal}}, a distributed RL framework specialized for applications in robotics.

==> text/challenges.tex <==
\
